TextBind: Multi-turn Interleaved Multimodal Instruction-following in the Wild

Large language models with instruction-following abilities have revolutionized the field of artificial intelligence. These models show exceptional generalizability to tackle various real-world tasks through their natural language interfaces. However, their performance heavily relies on high-quality exemplar data, which is often difficult to obtain. This challenge is further exacerbated when it comes to multimodal instruction following. We introduce TextBind, an almost annotation-free framework for empowering larger language models with the multi-turn interleaved multimodal instruction-following capabilities. Our approach requires only image-caption pairs and generates multi-turn multimodal instruction-response conversations from a language model. To accommodate interleaved image-text inputs and outputs, we devise MIM, a language model-centric architecture that seamlessly integrates image encoder and decoder models. We release our dataset, model, and demo to foster future research in the area of multimodal instruction following.

==> appx_human_data_analysis.tex <==
\section{Impact of Our Data \label{app:human_data_analysis}}
{

\color{red}{
\begin{table}[]
\begin{tabular}{l|lll}
\hline
 Model   & Instruction-following & Multi-modal Context Understanding & Informativeness \\ \hline
\textsc{LLaVA}    & 3.59                  & 3.56                              & 3.78            \\
\textsc{TextBind} & 3.99                  & 3.82                              & 3.72            \\ \hline
\end{tabular}\caption{Impact of our data. \label{tab:data_impact}}
\end{table}
}

}

